Optimal Quantization for Distribution Synthesis

Finite precision approximations of discrete probability distributions are considered, applicable for distribution synthesis, e.g., probabilistic shaping. Two algorithms are presented that find the optimal $M$-type approximation $Q$ of a distribution $P$ in terms of the variational distance $| Q-P|_1$ and the informational divergence $\mathbb{D}(Q| P)$. Bounds on the approximation errors are derived and shown to be asymptotically tight. Several examples illustrate that the variational distance optimal approximation can be quite different from the informational divergence optimal approximation.

==> proof.tex <==
 \section{Proofs}
\label{sec:proofs}

\subsection{Proof of Lemma~\ref{lem:IDboundVD}}
\label{sec:proof:idvdbound}
Define 
\begin{align}
\mathcal{A}:=\{i\colon p_i\geq t_i\},\quad P:=\sum_{i\in\mathcal{A}}p_i,\quad T:=\sum_{i\in\mathcal{A}}t_i. 
\end{align}
With this we express the variational distance as
\begin{align}
\lVert \vecp-\vect\rVert_1&=\sum_{i\in\mathcal{A}}(p_i-t_i)+\sum_{i\notin\mathcal{A}}(t_i-p_i)\nonumber\\
&=P-T+(1-T)-(1-P)\nonumber\\
&=2(P-T)=2\cdot\sum_{i\in\mathcal{A}}(p_i-t_i).\label{eq:vd2a}
\end{align}
Now,
\begin{align}
\kl(\vecp\Vert\vect)
&=\sum_{i\colon p_i>0}p_i\log\frac{p_i}{t_i}\\
&=\sum_{i\colon p_i>0}(p_i-t_i)\log\frac{p_i}{t_i}+\sum_{i\colon p_i>0}t_i\log\frac{p_i}{t_i}\\
&\stackrel{(a)}{\leq}\log r\sum_{i\colon p_i>0}(p_i-t_i)+\sum_{i\colon p_i>0}t_i\log\frac{p_i}{t_i}\\
&\leq\log r\sum_{i\colon p_i\geq t_i}(p_i-t_i)+\sum_{i\colon p_i>0}t_i\log\frac{p_i}{t_i}\\
&\stackrel{(b)}{=} \frac{1}{2}\log r\lVert \vecp-\vect\rVert_1+\sum_{i\colon p_i>0}t_i\log\frac{p_i}{t_i}\\
&\stackrel{(c)}{\leq} \frac{1}{2}\log r\lVert \vecp-\vect\rVert_1+\sum_{i\colon p_i>0}t_i\left(\frac{p_i}{t_i}-1\right)\\
&\leq \frac{1}{2}\log r\lVert \vecp-\vect\rVert_1+\sum_{i\colon p_i\geq t_i}(p_i-t_i)\\
&\stackrel{(d)}{=}\frac{1}{2}\log r\lVert \vecp-\vect\rVert_1+\frac{1}{2}\lVert \vecp-\vect\rVert_1\\
&=\frac{1}{2}\left(\log r+1\right)\lVert \vecp-\vect\rVert_1
\end{align}
where $(a)$ follows by the definition of $r$, $(b)$ and $(d)$ follow by \eqref{eq:vd2a} and where $(c)$ follows by $\log(x)\leq x-1$.
\endproof

\subsection{Proof of Lemma~\ref{lem:vdopt_quantBounds}}~\label{proof:vd:optprop}
We prove that every optimal $\vecp$ satisfies~\eqref{eq:quantBounds} by contradiction: Suppose that $|p_i-t_i|\ge\frac{1}{M}$ for some $i$. Thus, for some $k\in\mathbb{N}=\{1,2,\dotsc\}$, either $p_i=\frac{\lfloor Mt_i\rfloor-k}{M}$ or $p_i=\frac{\lceil Mt_i\rceil+k}{M}$. We treat only the first case, the second follows along the same lines. Recognize that
\begin{equation}
 p_i=\frac{\lfloor Mt_i\rfloor-k}{M}
\Rightarrow \exists j\colon \exists m\in\mathbb{N}\colon p_j = \frac{\lfloor Mt_j\rfloor+m}{M}
\end{equation}
because the entries of $\vecp$ must sum up to one. Second, let $\vecp^\circ$ be such that $p_i^\circ=p_i+\frac{1}{M}$, $p_j^\circ = p_j-\frac{1}{M}$, and $p_\ell^\circ=p_\ell$ for all $\ell\neq i,j$. We calculate
\begin{align}
\lVert\vecp-\vect\rVert_1-\lVert\vecp^\circ-\vect\rVert_1
&=t_i-p_i-t_i+p_i^\circ+p_j-t_j-|p_j^\circ-t_j| \notag\\
&=\frac{1}{M}+p_j-t_j-|p_j^\circ-t_j|.\label{eq:vdproof:lastline}
\end{align}
For $m>1$ one obtains $p_j^\circ>t_j$ and~\eqref{eq:vdproof:lastline} evaluates to $\frac{2}{M}>0$. For $m=1$, continuing with \eqref{eq:vdproof:lastline} yields
\begin{align}
\lVert\vecp-\vect\rVert_1-\lVert\vecp^\circ-\vect\rVert_1
&=\frac{1}{M}+p_j+p_j^\circ-2t_j\notag\\
&=\frac{2\lfloor Mt_j\rfloor+2}{M}-2t_j>0.
\end{align}
We conclude that an optimal algorithm cannot violate~\eqref{eq:quantBounds}.

To prove that every optimal $\vecp$ satisfies Lemma~\ref{lem:firstM_vd} requires to look into the proof of Proposition~\ref{prop:vdopt}. From there, it can be seen that the cost in terms of variational distance would be strictly larger if Lemma~\ref{lem:firstM_vd} is violated for a pair $i,j$ with the given assumptions.
\endproof


\subsection{Proof of Lemma~\ref{lem:subprobability}}
\label{sec:proof:lem}
\input{proof_lem}

\subsection{Proof of Proposition~\ref{prop:vdbounds}}
\label{sec:proof:vd}
\input{proof_vd}

\subsection{Proof of Lemma~\ref{lem:ratiobound}}
\label{sec:proof:ratiobound}
 Recall $\qtid_i=\frac{c_i}{M}$ and suppose entry $i$ got assigned the $c_i$-th unit mass in some iteration when entry $1$ has pre-allocation $\tilde{c}_1$. Then 
\begin{align}
\Delta_i(c_i)\leq\Delta_1(\tilde{c}_1+1)\leq\Delta_1(M).
\end{align}
We bound the term on the right-hand side.
\begin{align}
\Delta_1(M)&=M\log\frac{M}{t_1}-(M-1)\log\frac{M-1}{t_1}\\
&=\log\frac{M}{t_1}+(M-1)\log\frac{M}{M-1}\\
&=\log\frac{M}{t_1}+(M-1)\log\left(1+\frac{1}{M-1}\right)\\
&< \log\frac{M}{t_1}+1\\
&=\log\frac{Me}{t_1}.
\end{align}
In a similar way we bound $\Delta_i(c_i)$ from below. We have
\begin{align}
\Delta_i(c_i)&=c_i\log\frac{c_i}{t_i}-(c_i-1)\log\frac{c_i-1}{t_i}\\
&=\log\frac{c_i}{t_i}+(c_i-1)\log\frac{c_i}{c_i-1}\\
&> \log\frac{c_i}{t_i}.
\end{align}
Thus
\begin{align}
\log\frac{c_i}{t_i}< \log\frac{Me}{t_1}\Rightarrow \frac{c_i}{Mt_i}=\frac{\qtid_i}{t_i}< \frac{e}{t_1}.
\end{align}
The particular result for index $k$ results from $\qtid_k\ge 1/M$.


\subsection{Proof of Proposition~\ref{prop:idopt}}
\label{sec:proof:idopt}
\input{proof_id_opt}


\subsection{Proof of Proposition~\ref{prop:idbounds}}
\label{sec:proof:id}
\input{proof_id}


==> proof_id_opt.tex <==

To prove optimality, we need the following lemma:
\begin{lemma}\label{lem:bounded}
Let $\vecc^*$ be an optimal allocation. Let $\vecc$ be a pre-allocation with $\sum_ic_i<M$ and $c_i\leq c^*_i$ for $i=1,\dotsc,n$. Define
\begin{align}
j=\argmin_i\Delta_i(c_i+1).\label{eq:defj}
\end{align}
Then there exists an optimal allocation $\tilde{\vecc}$ with
\begin{align}
c_j+1&\leq \tilde{c}_j\label{eq:lem2:statement}\\
c_i&\leq\tilde{c}_i,\quad i=1,\dotsc,n.
\end{align}
\end{lemma}
\begin{proof}
Suppose we have
\begin{align}
c_j+1>c^*_j.\label{eq:lem2:supp}
\end{align}
Since $c_j\leq c^*_j$ by assumption, \eqref{eq:lem2:supp} implies
\begin{align}
c_j+1=c^*_j+1.\label{eq:lem2:prop1}
\end{align}
Since $\sum_ic_i<M$ and $\sum_ic^*_i=M$, there must be at least one $\ell\neq j$ with
\begin{align}
c^*_\ell\geq c_\ell+1.\label{eq:lem2:prop2}
\end{align}
By decreasing $c^*_\ell$ by one and increasing $c^*_j$ by one, the change of the objective function is $\Delta_j(c^*_j+1)-\Delta_\ell(c^*_\ell)$. We bound this change as follows.
\begin{align}
\Delta_j(c^*_j+1)-\Delta_\ell(c^*_\ell)&\overset{\text{(a)}}{\leq} \Delta_j(c^*_j+1)-\Delta_\ell(c_\ell+1)\label{eq:lem1:neq1}\\
&\overset{\text{(b)}}{=} \Delta_j(c_j+1)-\Delta_\ell(c_\ell+1)\\
&\overset{\text{(c)}}{\leq} \label{eq:lem1:neq2}0
\end{align}
where (a) follows by \eqref{eq:lem2:prop2} and Lemma~\ref{lem:ifproperties}, (b) follows by \eqref{eq:lem2:prop1}, and (c) follows by the definition of $j$ in \eqref{eq:defj}.

We have to consider two cases. First, suppose we have strict inequality in either \eqref{eq:lem1:neq1} or \eqref{eq:lem1:neq2}. Then the objective function is decreased, which contradicts the assumption that $\vecc^*$ is optimal. Thus, the supposition \eqref{eq:lem2:supp} is false and the statements of the lemma hold for $\tilde{\vecc}=\vecc^*$. Second, suppose we have equality both in \eqref{eq:lem1:neq1} and \eqref{eq:lem1:neq2}. In this case, define the allocation
\begin{align}
\tilde{c}_\ell = c^*_\ell-1,\quad\, \tilde{c}_j = c^*_j + 1,\quad\, \tilde{c}_i = c^*_i\text{ for } i\neq j,\ell.
\end{align}
Equality in \eqref{eq:lem1:neq1}--\eqref{eq:lem1:neq2} implies optimality of $\tilde{\vecc}$. By \eqref{eq:lem2:prop1} and \eqref{eq:lem2:prop2}, we can verify that $\tilde{\vecc}$ fulfills the statements of the lemma. This concludes the proof.
\end{proof}
By Lemma~\ref{lem:bounded}, there is an optimal allocation $\tilde{\vecc}$ such that in each iteration of Algorithm~\ref{alg:id} we have 
\begin{align}
c_i\leq \tilde{c}_i,\qquad i=1,\dotsc,n.\label{eq:proof1}
\end{align}
After termination of Algorithm~\ref{alg:id}, we have
\begin{align}
M=\sum_i c_i \leq \sum_i \tilde{c}_i = M.\label{eq:proof2}
\end{align}
Statements \eqref{eq:proof1} and \eqref{eq:proof2} can only be true simultaneously if $c_i= \tilde{c}_i$ for all $i=1,\dotsc,n$. Consequently, the constructed allocation $\vecc$ is optimal. This concludes the proof.

==> proof_lem.tex <==
Algorithm~\ref{alg:vd} can have two different results: If $T_k > k/M$, one has
\begin{equation}
 T_k = 1-\sum_{i=1}^k t_i = \sum_{i=1}^k \qtvd_i-t_i >\frac{k}{M}.
\end{equation}
But the algorithm cannot at the same time have $\qtvd_i-t_i>1/M$ and $\qtvd_j-t_j<0$ for $i,j\in\{1,\dots,k\}$, $i\neq j$. Hence, in order that above equation is satisfied, $\qtvd_i-t_i>0$ for all $i$, and thus
\begin{equation}
 \lVert\vecqtvd-\vect\rVert_1 = \sum_{i=1}^k |\qtvd_i-t_i| = \sum_{i=1}^k \qtvd_i-t_i = T_k.
\end{equation}

If $T_k<k/M$, then either are all differences $\qtvd_i-t_i>0$ (with some even being larger than $1/M$) or some differences are positive and some are negative. In the former case, $\lVert\vecqtvd-\vect\rVert_1 = T_k$. In the latter, the algorithm guarantees that~\eqref{eq:quantBounds} holds.

By definition of the rest mass,
\begin{equation}
 1-\frac{L}{M} = \sum_{i=1}^k \frac{\lfloor Mt_i\rfloor}{M} = \sum_{i=1}^k t_i-e_i
\end{equation}
from which follows that
\begin{equation}
 \sum_{i=1}^k e_i = \frac{L}{M}-T_k.
\end{equation}
Reorder now the first $k$ errors such that $\tilde{e}_i\ge\tilde{e}_{i+1}$. Thus, we can bound the mean error from below and above by
\begin{equation}
 \frac{1}{L} \sum_{i=1}^L \tilde{e}_i \ge \frac{L}{Mk}-\frac{T_k}{k} \ge \frac{1}{k-L}\sum_{i=L+1}^k \tilde{e}_i. \label{eq:vdproof:inequality}
\end{equation}
Equality holds if $\tilde{e}_i=\frac{L}{Mk}-\frac{T_k}{k}$ for all $i=1,\dots,k$. With these inequalities we obtain
\begin{align}
 \sum_{i=1}^k |t_i-\qtvd_i|
&= \sum_{i=1}^L \left(\frac{1}{M}-\tilde{e}_i\right) + \sum_{i=L+1}^k \tilde{e}_i\\
&\le \frac{L}{M} + \left(\frac{L}{Mk}-\frac{T_k}{k}\right)(k-2L).
\end{align}
The maximum is achieved for $L=(k+MT_k)/2$, which yields
\begin{equation}
 \lVert\vecqtvd-\vect\rVert_1 \le \frac{k}{2M}+\frac{MT_k^2}{2k}.
\end{equation}
Thus, for $T_k<k/M$, one has
\begin{equation}
 \lVert\vecqtvd-\vect\rVert_1 \le \max\left\{T_k, \frac{k}{2M}+\frac{MT_k^2}{2k}\right\}.
\end{equation}
Since the latter is always larger than the former for this case, the proof for the better of the two bounds is completed. The proof for the worse one is omitted.\endproof
